Optimization of Hybrid Power Plants: When Is a Detailed Electrolyzer Model Necessary?

Hybrid power plants comprising renewable power sources and electrolyzers are envisioned to play a key role in accelerating the transition towards decarbonization. It is common in the current literature to use simplified operational models for electrolyzers. It is still an open question whether this is a good practice, and if not, when a more detailed operational model is necessary. This paper answers it by assessing the impact of adding different levels of electrolyzer details, i.e., physics and operational constraints, to the optimal dispatch problem of a hybrid power plant in the day-ahead time stage. Our focus lies on the number of operating states (on, off, standby) as well as the number of linearization segments used for approximating the non-linear hydrogen production curve. For that, we develop several mixed-integer linear models, each representing a different level of operational details. We conduct a thorough comparative ex-post performance analysis under different price conditions, wind farm capacities, and minimum hydrogen demand requirements, and discuss under which operational circumstances a detailed model is necessary. In particular, we provide a case under which a simplified model, compared to a detailed one, results in a decrease in profit of 1.8% and hydrogen production of 13.5% over a year. The key lesson learned is that a detailed model potentially earns a higher profit in circumstances under which the electrolyzer operates with partial loading. This could be the case for a certain range of electricity and hydrogen prices, or limited wind power availability. The detailed model also provides a better estimation of true hydrogen production, facilitating the logistics required.

==> 1_Nomenclature.tex <==
\section*{Nomenclature}

\subsection{Sets}
\begin{table}[h!]
\begin{tabular}{lll}
    $A$ & Set of hydrogen production slopes & [kg/MWh] \\
    $B$ & Set of hydrogen production intercepts & [kg] \\
    $S$ & Number of production segments & [--] \\
    $T$ & Set of time steps & [h]
\end{tabular}
\end{table}

\subsection{Parameters}
\begin{table}[h!]
\begin{tabular}{lll}
    $C^W$ & Wind farm capacity & [MW] \\
    $C^E$ & Electrolyzer capacity & [MW] \\
    $P^W_t$ & Wind production & [MWh] \\
    $\overline{P}^{E}$ & Maximum electrolyzer load & [MW] \\
    $\underline{P}^{E}$ & Minimum electrolyzer load & [MW] \\
    $P^{sb}$ & Standby electrolyzer load & [MW] \\
    $\lambda^M_t$ & Electricity market price & [EUR/MWh] \\
    $\lambda^H$ & Hydrogen market price & [EUR/MWh] \\
    $\lambda^{start}$ & Electrolyzer start-up cost & [EUR/MW]
\end{tabular}
\end{table}

\subsection{Variables}
\begin{table}[h!]
\begin{tabular}{llll}
    $e_t $&$ \in \mathbb{R}^+$ & Electrolyzer consumption & [MWh] \\
    $h_t $&$ \in \mathbb{R}^+$ & Hydrogen production & [kg] \\
    $m_t $&$ \in \mathbb{R}^+$ & Electricity sold in time step & [MWh] \\
    $z^{h}_{t,s} $&$ \in \{0,1\}$ & Production segment chosen if 1 & [--] \\
    $z^{on}_t $&$ \in \{0,1\}$ & Electrolyzer is on if 1 & [--] \\
    $z^{off}_t $&$ \in \{0,1\}$ & Electrolyzer is off if 1 & [--] \\
    $z^{sb}_t $&$ \in \{0,1\}$ & Electrolyzer is in standby if 1 & [--] \\
    $z^{start}_t $&$ \in \{0,1\}$ & Electrolyzer starts if 1 & [--]
\end{tabular}
\end{table}

==> Authors.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Manuel Tobias Baumhof }
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}

==> code_not_used.tex <==
Reversible cell voltage
\begin{align}
    U_{rev} = a_1 - a_2 T_K + a_3 T_K \text{ln}(T_K) + a_4 {T_K}^2 \label{eq:U_rev}
\end{align}

Faraday efficiency
\begin{align}
    \eta_{F} = B_1 + B_2 \text{exp} \left( \frac{B_3 + B_4 T_{C} + B_5 T^2}{i} \right) \label{eq:faraday}
\end{align}

\begin{table}[h!]
    \centering
    \caption{Chosen input parameter for operation.}
        \begin{tabular}{crl}
        \hline
        \textbf{Parameter} & \textbf{Value} & \textbf{Unit} \\ \hline
        $\text{i}_{\text{max}}$ & 5000 & A $\text{m}^{-2}$ \\
        T & 80 & $^{\circ}\text{C}$ \\
        $\text{T}_{\text{K}}$ & 353.15 & K \\
        p & 30 & bar \\ \hline
        \end{tabular}
    \label{tab:param}
\end{table}


\subsubsection{Hydrogen storage}
%The model can be extended to include storage and hydrogen demand. 
The hydrogen produced $h_t$ can either go directly to the demand $h^{\rm{d}}_t$ or be injected into the hydrogen storage $s^{\rm{in}}_t$, therefore
\begin{align}
    & h_t = h^{\rm{d}}_t + s^{\rm{in}}_t & \forall~ & t \in \mathcal{T}. \ \label{eq:stor_1}
\end{align}
Further, the total hydrogen $d_t$ to be delivered is equal to the sum of hydrogen directly to the demand and from the storage $s^{\rm{out}}_t$, i.e.,  
\begin{align}
    & d_t = h^{\rm{d}}_t + s^{\rm{out}}_t & \forall~ & t \in \mathcal{T}.
\end{align}
The storage output of every hour is limited by the output flow capacity $S^{\rm{out}}$ as
\begin{align}
    & s^{\rm{out}}_t \leq S^{\rm{out}} & \forall~ & t \in \mathcal{T}. \
\end{align}
In addition, the compressor consumes power $p^{\rm{c}}$ to compress the hydrogen injected into the storage. Assuming adiabatic compression, the compression coefficient $K^{\rm{c}}$ can be calculated, as proposed by \cite{ShiYou}. The power consumption for compression is then: 
\begin{align}
    & p^{\rm{c}}_t = K^{\rm{c}} s^{\rm{in}}_t & \forall~ & t \in \mathcal{T}.
\end{align}
%The state of the storage is tracked based on the state in the previous time step, and the input and output of the present time step. 
The state of charge of the hydrogen storage in the initial and following hours is calculated by
%The storage has a maximum capacity given by $C^{\rm{s}}$.
\begin{align}
    & s_{t=1} = S^{\rm{ini}} + s^{\rm{in}}_{t=1} - s^{\rm{out}}_{t=1} &  \\
    & s_t = s_{t-1} + s^{\rm{in}}_t - s^{\rm{out}}_t & \forall~ & t \in \mathcal{T} \backslash 1, \
\end{align}
where $S^{\rm{ini}}$ is the hydrogen initially stored in the storage at the beginning of time horizon $\mathcal{T}$.
The storage hydrogen mass capacity $C^{\rm{s}}$ is enforced by
%The storage has a maximum capacity given by $C^{\rm{s}}$.
\begin{align}
    & s_t \leq C^{\rm{s}} & \forall~ & t \in \mathcal{T}. \label{eq:stor_2}
\end{align}

Note that we do not impose any constraint for the energy stored at the end of time horizon $\mathcal{T}$. Therefore, pursuing profit maximization in this time horizon, the hybrid power plant will leave the storage empty in the last hour\footnote{One can enforce a constraint on the minimum stored hydrogen at the end of the time horizon, or add a value for this stored energy to the objective function.}.
